Understanding Natural Language Instructions for Fetching Daily Objects Using GAN-Based Multimodal Target-Source Classification

In this paper, we address multimodal language understanding for unconstrained fetching instruction in domestic service robots context. A typical fetching instruction such as "Bring me the yellow toy from the white shelf" requires to infer the user intention, that is what object (target) to fetch and from where (source). To solve the task, we propose a Multimodal Target-source Classifier Model (MTCM), which predicts the region-wise likelihood of target and source candidates in the scene. Unlike other methods, MTCM can handle regionwise classification based on linguistic and visual features. We evaluated our approach that outperformed the state-of-the-art method on a standard data set. In addition, we extended MTCM with Generative Adversarial Nets (MTCM-GAN), and enabled simultaneous data augmentation and classification.

==> tex/label.tex <==
 \section{ multi-modal data set}\label{sec:label}
 In this section, we detail the construction of our dataset. As mentioned in Section X, this dataset has been collected from the virtual environment SIGVerse \cite{inamura2013development}. This choice allows to generalize our approach by considering various environment setups, which would be difficult and tedious in real-world situation.
\subsection{Overview of the Data Set Construction}\label{sec:data_constr}

First, an overview of the different steps to build are detailed below. Each of these steps are subsequently more thoroughly detailed in the next sections

\begin{itemize}
\item[$1$.] Run a given simulation environment on SIGVerse 
\item[$2$.] Take snapshots of the environments at different key spots
\item[$3$.] Instruct a first labeler to write a natural fetching instruction based on $2$ and according to the context.
%\item[$4$.] Instruct a second labeler to put a class label on each object according to the instruction given in $3$.
\end{itemize} 
\Done

 \subsection{About SIGVerse} \label{sec:sigverse}
 Currently, SIGVerse is used for several robotics competition. Another benefit is that SIGVerse is also used in robotics competitions, Robocup@Home or more recently for World Robot Summit (WRS)  partner service robot challenges. In particular one of the tasks in WRS, HandyMan, is about understanding fetching instructions. Typical instructions mentioning a location, an object and a destination are given to the robot that should explore the environment, grasp the correct object and place it in the correct location. Hence, SIGVerse provides an adequate simulation environment for the purpose of our initial task, since the purpose of Handyman task is very similar to the problem addressed in this paper.  However, while the placing task has been previously addressed in \cite{magassouba2018multimodal}, we want to tackle the fetching task in a more intuitive and natural way. Indeed, unlike Handyman task, we do not constraint the instruction format. No specific structure nor keyword should be used to command the robot. 


\subsection{Image data collection method}
We collected images from the robot during the exploration phases of the robot in several environments. To refer to our main reason to use SIGVerse, each environment has different setups: different rooms in number and types coupled with different furniture configuration. In total we used 4 environments. We ran this exploration phase 3 times in each environment, with random objects positions every time. During this process, the images recorded from head cameras are saved. We could collect more than 5000 images. Among them, we selected only the valid images for our task. More specifically, a given image is considered valid only if it contains one or several pieces of furniture and visible objects on them. From this procedure, we used XXXX valid images.

In a second phase, through a specifically trained YOLO \cite{redmon2016you} image detection model, we could retrieve all bounding boxes related to each object and piece of furniture,  as shown in Fig. X. Thereafter, these bounding boxes were manually reviewed  and corrected when required.


\subsection{Labeling image data}
The second input of our system consists in the linguistic data. Each object in a given scene should be associated with one or several instructions characterizing a fetching task. The instructions were given only for the candidate objects not to pieces of furniture.

A non expert labeler was then instructed to give a natural fetching instruction related to each candidate object in the scene.  For each object several type of instructions can be assumed. We divided the instructions into two sets described as follow:
\begin{itemize}
    \item $I_{F}$: The instruction should contain a candidate piece of furniture $F$, e.g., ``Bring me the coke bottle that is on the table''
    \item $I_{N}$: The instruction should not contain any candidate piece of furniture, e.g., ``Pick up the coke and bring it to me''
\end{itemize} 

 \begin{figure}[b]
   \centering
      \includegraphics[scale=0.45]{data.png}
      \caption{\small Samples of the $1282$ depth images (right) ${\bf v}_d$ and their corresponding RGB images (left). Only the depth data is used.}
   \label{fig:data}
   \squeezeup
 \end{figure}

 
\begin{table}[t]
\normalsize
\caption{\small Data collection statistics }
\label{tab:data_coll}
\centering
\begin{tabular}{lccc}
\hline
$\#$ &Instance &Target areas &Images\\
\hline
Table &4&18&321 \\
  
Drawer &4 &10&336\\

Desk&4&8&425 \\

Shelf&2&5&200 \\
\hline
$\sum$ &{\bf 14}& {\bf 37}& {\bf 1282}\\
\hline
\end{tabular}
    \squeezeup
   \squeezeup

\end{table}


 \begin{figure}[tp]
   \centering
      \includegraphics[scale=0.4]{feature.png}
      \caption{\small Example of multimodal input composed of a depth image ${\bf v}_d$ and the associated meta-data ${\bf v}_{meta}$ (camera height, target height, camera angle) with the instruction ${\bf w}_{inst}$ and context ${\bf w}_{c}$.}
   \label{fig:features}
   \squeezeup
   \squeezeup
  \end{figure} 
  
 \subection{relational features}
 As discussed before since the relational features ca, we define the relational features used for each task.

\subsection{Labeling Strategy}\label{sec:labeling}
After giving the instructions, each object is manually labeled into categories by a robotic expert. These categories refer to the likelihood of the object corresponding to the instruction. 

\Update
We then define four class categories that characterize the likelihood of a candidate object, given an instruction. These categories are given as :

\begin{itemize}
\item[($A1$)]  The candidate object $O_i$ is very likely in terms of linguistic and visual information %The robot is highly likely to accomplish the instruction.
\item[($A2$)]  The candidate object $O_i$ is likely in terms of linguistic and visual information: this label is used when the target object is not explicitly given in the instruction (e.g. ``Bring me the black and red object from the table '')
\item[($A3$)] The  candidate object $O_i$   is unlikely in terms of linguistic and/or visual information: The candidate object does not correspond to the description. 
\item[($A4$)] The  candidate object $O_i$ is very unlikely in terms of linguistic and/or visual information: The object does not correspond to the description and/or does not  belong to the specified piece of furniture . %The instruction cannot be performed  by the robot.
\end{itemize}  
\Done


Thereafter the dataset was randomly  split into training, validation and test sets as described in Table \ref{tab:data_table}.


\begin{table}[h]
\normalsize
\caption{\small Statistics of the data set ${\bf x}_{real}$}
\label{tab:data_table}
\centering
\begin{tabular}{cccc|c }
\hline
$\#$ & Train& Valid& Test& $\sum$\\
\hline
$A1$  &158&29&25&{\bf 212} \\

$A2$&359&34&39&{\bf 432}\\

$A3$&350&26&22 &{\bf 398}  \\

$A4$&203&17&20 & {\bf 240}\\
\hline
$\sum$& {\bf 1070} ({\it 83 $\%$}) & {\bf 106} ({\it 8.5 $\%$}) & {\bf 106} ({\it 8.5 $\%$}) & \multicolumn{1}{ |c}{\bf 1282}\\
\hline
\squeezeup
\squeezeup
\squeezeup
\end{tabular}
\end{table}






















